Sum-max Submodular Bandits

Many online decision-making problems correspond to maximizing a sequence of submodular functions. In this work, we introduce sum-max functions, a subclass of monotone submodular functions capturing several interesting problems, including best-of-$K$-bandits, combinatorial bandits, and the bandit versions on facility location, $M$-medians, and hitting sets. We show that all functions in this class satisfy a key property that we call pseudo-concavity. This allows us to prove $\big(1 - \frac{1}{e}\big)$-regret bounds for bandit feedback in the nonstochastic setting of the order of $\sqrt{MKT}$ (ignoring log factors), where $T$ is the time horizon and $M$ is a cardinality constraint. This bound, attained by a simple and efficient algorithm, significantly improves on the $\widetilde{O}\big(T^{2/3}\big)$ regret bound for online monotone submodular maximization with bandit feedback.

==> intro-old.tex <==
\section{Introduction}

In this paper we give an algorithm for online cardinality-constrained set-function maximisation under bandit feedback. In this problem we have a set of $\nmb$ \emph{arms} and on any trial $t$ must choose a subset $\cho{t}$ of at most $\siz$ arms. On such a trial $t$ there exists an unknown set function $\ret{t}$. After the choice of $\cho{t}$ we are rewarded by $\ret{t}(\cho{t})$. We note that the only feedback that we recieve is the value $\ret{t}(\cho{t})$. Our aim is to maximise the cumulative reward:
\be
\sum_{t\in[\ntr]}\ret{t}(\cho{t})
\ee
In this paper we give an algorithm \alg\ (Multiple Sample \textsc{Exp3}) for solving this problem.  \alg\ is extremely efficient - having a per-trial time complexity of only $\mathcal{O}(\siz\ln(\nmb))$ when implemented with a binary tree over the arms as in \cite{}.

Of course, if each reward function $\ret{t}$ is completely unconstrained then the problem becomes identical to the adversarial bandit problem with $\Omega(\nmb^{\siz})$ arms leading to a massive regret. Hence, we will give performance guarantees for \alg\ for a specific, but very general, class of reward functions. Specifically, we restrict our attention to \emph{pseudo-concave pseudo-submodular} functions defined as follows:

\begin{definition}\label{qcdef}
Suppose we have a set function $\af:2^{[\nmb]}\rightarrow\br$. For any $\ass\subseteq[\nmb]$ define the matrix $\mat{\af}{\ass}\in\br^{\nmb\times\nmb}$ such that for all $i,j\in[\nmb]$ we have:
\be
\mac{\af}{\ass}{i}{j}:=\af(\ass\cup\{i,j\})
\ee
We call the function $\af$ \emp{pseudo-concave} if and only if for all $\ass\subseteq[\nmb]$ and all $\ave\in\br^{\nmb}$ with $\ave\cdot\bs{1}=0$ we have:
\be
\tra{\ave}\mat{\af}{\ass}\ave\leq0
\ee
\end{definition}

\begin{definition}\label{pssubdef}
A set function $\af:2^{[\nmb]}\rightarrow\br$ is \emp{pseudo-submodular} if and only if for every set $\ass\subseteq[\nmb]$ with $\ass\neq\emptyset$ there exists some $i\in\ass$ such that for all $\bas\subseteq\ass\setminus\{i\}$ we have:
\be
\af(\bas\cup\{i\})-\af(\bas)\geq\af(\ass)-\af(\ass\setminus\{i\})
\ee
\end{definition}
We note that all submodular set functions are pseudo-submodular. We will later give real-world examples of pseudo-concave pseudo-submodular set functions. In particular, we show that \alg\ solves the online learning version of the $\siz$-medians problem with fully-bandit feedback.

In many real world problems the choice of each arm $i$ on some trial $t$ invokes a cost (i.e. negative reward) $\ctc{t}{i}$. When this is the case we would like to maximise the cumulative profit:
\be
\sum_{t\in[\ntr]}\left(\ret{t}(\cho{t})-\sum_{i\in\cho{t}}\ctc{t}{i}\right)
\ee
We will show that \alg\ can handle this generalised problem if it recieves, at the end of each trial $t$, the values of $\ctc{t}{i}$ for all $i\in\cho{t}$. We note that the fully bandit \alg\ without costs is a special case of \alg\ with costs. The inclusion of costs will allow us to solve, as an example, the online learning version of the \emph{facility location problem} with semi-bandit feedback. Both this problem and the $\siz$-median problem have important applications in advertising and cyber-security.

\textcolor{red}{NCB} Our main result implies a $\mathcal{O}\big(\sqrt{M\nmb(\ln(\nmb)T}\big)$ bound on the $\gamma$-regret for some $\gamma < 1-\frac{1}{e}$ when we have no costs. For comparison, the optimal approximation factor for submodular maximization with cardinality constraints is $\frac{1}{2}$, whereas $1-\frac{1}{e}$ is optimal only in the monotone submodular case. When $M=1$ we recover the adversarial $\nmb$-armed bandit problem. In this case $\gamma =1$ and our bound specializes to the standard $\mathcal{O}\big(\sqrt{\nmb\ln (\nmb)T}\big)$ regret bound of \textsc{Exp3}. In fact, when $M=1$ and there are no costs, our algorithm \alg\ is identical to \textsc{Exp3}. \alg\ can hence be seen as a generalisation of \textsc{Exp3}.

==> lowerapprox.tex <==
\section{Approximation Ratio}

\nc{\apr}{\alpha}
\nc{\tpo}{s}
\nc{\lgt}{\log_2}
\nc{\rct}{c}
\nc{\ses}{K}
\nc{\cov}[1]{\mathcal{C}_{#1}}
\nc{\bet}[1]{\beta_{#1}}
\nc{\mco}{\mathcal{S}}
\nc{\cco}{\gamma}
\nc{\sca}{\epsilon}
\nc{\bprob}[1]{\mathbb{P}\left[#1\right]}
\nc{\prp}{s}
\nc{\mmu}{c}
\nc{\kex}{d}
\nc{\raf}{g}
\nc{\haf}{h}
\nc{\ssi}{n}
\nc{\kld}[2]{\delta(#1,#2)}

We now show that, for the clickthrough model, the approximation ratio of $1-\alpha^\siz$ is necessary for any polynomial time algorithm unless there exist an efficient algorithm for the set cover problem on $[\nmb]$ with an approximation ratio better than $\ln(\nmb)$.
%
\begin{theorem}\label{Th:LB1}
Pick any $\nid\in\nat$. If there exists some $\kex\in\nat$, $\tpo\in(0,1)$, $\cco > 1$, $\sca \in (1/\cco,1)$, and a randomized polynomial time algorithm for Learner such that:
\be
\bexpt{\sum_{t\in[\ntr]}\ret{t}(\cho{t})}\geq\left(1-\left(\frac{|\ars|-1}{|\ars|}\right)^{\cco\siz}\right)\sum_{t\in[\ntr]}\ret{t}(\ars)- \mathcal{O}(\nid^\kex\ntr^\tpo)
\ee
for any subset $\mco$ of $[\nid]$ and for any $\siz\in\nat$,
then, for all $\ssi>4^{1/(\sca\cco-1)}$, there exists a randomized polynomial-time algorithm for the set cover problem on $[\ssi]$ that, with probability at least $\frac{1}{2}$, achieves approximation ratio at least $\sca\ln(\ssi)$.
\end{theorem}

\begin{proof}
Suppose we have such an algorithm. Let $\rct>0$ and $\cco>1$ be such that:
\begin{equation}\label{arbeq2}
\bexpt{\sum_{t\in[\ntr]}\ret{t}(\cho{t})}\geq\left(1-\left(\frac{|\ars|-1}{|\ars|}\right)^{\cco\siz}\right)\sum_{t\in[\ntr]}\ret{t}(\ars)- \rct\nid^\kex\ntr^\tpo
\end{equation}
Choose any $\sca\in(1/\cco,1)$ and then consider any $\ssi\in\nat$ such that $\ssi>4^{1/(\sca\cco-1)}$. Consider also any collection of sets $\{\cov{k}~|~k\in[\nid]\}\subseteq2^{[\ssi]}$ such that: 
\be
\bigcup_{k\in[\nid]}\cov{k}=[\ssi]
\ee
Let $\mco$ be a subset of $[\nid]$ of minimum cardinality such that:
\be
\bigcup_{k\in\mco}\cov{k}=[\ssi]
\ee
Now choose: 
\be
\ntr:=\left\lceil(4\rct\nid^{\kex}\ssi)^{1/(1-\tpo)}\right\rceil
\ee 
and choose any $\siz\in\nat$ such that $\siz\geq\sca\ln(\ssi)|\ars|$. For all $t\in[\ntr]$ draw $\aws{t}$ randomly as follows. First draw $\bet{t}$ uniformly at random from $[\ssi]$ and then define:
\be
\aws{t}:=\{k\in[\nid]~|~\bet{t}\in\cov{k}\}
\ee
It is a classic result that:
\be
\left(\frac{|\ars|-1}{|\ars|}\right)^{|\ars|}\leq e^{-1}
\ee
so by the conditions on $\ssi$ and $\siz$ we have:
\begin{equation}\label{arbeq3}
\left(\frac{|\ars|-1}{|\ars|}\right)^{\cco\siz}\leq\exp(-\cco\siz/|\ars|)=\ssi^{-\sca\cco}=\frac{\ssi^{1-\sca\cco}}{\ssi}<\frac{1}{4\ssi}
\end{equation}
By definition of $\mco$ we have, for all $t\in[\ntr]$, that there exists some $k\in\mco$ such that $\bet{t}\in\cov{k}$ so that $\aws{t}\cap\mco\neq\emptyset$. This implies:
\be
\sum_{t\in[\ntr]}\ret{t}(\ars)=\ntr
\ee
and hence, by~\eqref{arbeq2} and~\eqref{arbeq3}, we have:
\begin{equation}\label{arbeq1}
\bexpt{\sum_{t\in[\ntr]}(1-\ret{t}(\cho{t}))}\leq\ntr-\ntr+\frac{\ntr}{4\ssi}+\rct\nid^\kex\ntr^\tpo\leq \frac{\ntr}{4\ssi} +\frac{\ntr\rct\nid^\kex}{\ntr^{1-\tpo}}\leq\frac{\ntr}{2\ssi}
\end{equation}
Fix $t$ and a realization of $\cho{t}$. If we have:
\be
\bigcup_{k\in\cho{t}}\cov{k}\neq[\ssi]
\ee
then we must also have that:
\begin{align*}
    \expt{1-\ret{t}(\cho{t}) \mid \cho{t}}
&=
    \prob{\cho{t}\cap\aws{t}=\emptyset \mid \cho{t}}
\\ &=
    \prob{\forall\, k\in\cho{t}\,,\,\bet{t}\notin\cov{k} \mid \cho{t}}
\\ &=
    \bprob{\left.\bet{t}\notin\bigcup_{k\in\cho{t}}\cov{k} \,\right\vert\, \cho{t}}
\ge
    \frac{1}{\ssi}    
\end{align*}
%so that:
%\be
%\bexpt{\sum_{t\in[\ntr]}(1-\ret{t}(\cho{t}))}\geq \frac{\ntr}{\ssi}
%\ee
Hence, by taking the randomness of $\cho{1},\ldots,\cho{T}$ into account,
\begin{align*}
    &\bprob{\sum_{t\in[\ntr]} \indi{\bigcup_{k\in\cho{t}}\cov{k}\neq[\ssi]} = T}
\\ &\le
    \bprob{\bexpt{\left.\sum_{t\in[\ntr]} \big(1-\ret{t}(\cho{t})\big) \,\right\vert\, \cho{1},\ldots,\cho{T}} \ge \frac{T}{n}}
\le
    \frac{1}{2}
\end{align*}
by \eqref{arbeq1}.
Since $\ntr$ is polynomial in $\nid\ssi$ and $|\cho{t}|\leq\siz$, we have a randomized polynomial-time algorithm that, with probability at least $\frac{1}{2}$, solves the set cover problem on $[\ssi]$ with approximation ratio $\sca\ln(\ssi)$ for $\sca \in (0,1)$.
\end{proof}


==> mse3.tex <==
\subsection{How and why \alg\ works}

We first give an overview of how \alg\ works when we have no costs (i.e. $\ctc{t}{i}=0$). \alg\ works by maintaining a probability distribution over the set of arms. Specifically, $\pvt{t}\in\splx{\nmb}$ is the vector whose components are the probabilities of drawing the actions on trial $t$. On trial $t$ the algorithm constructs the set $\cho{t}$ by drawing a sequence $\langle\acc{t}{j}\,|\,j\in[\siz]\rangle$ of arms i.i.d. with replacement from $\pvt{t}$ and then setting $\cho{t}=\{\acc{t}{j}\,|\,j\in[\siz]\}$.

Hence, for all set functions $\af$ we will construct a function $\phr{\af}:\mathbb{R}_+^{\nmb}\rightarrow\mathbb{R}$ such that for all $\apv\in\splx{\nmb}$ we have that $\phr{\af}(\apv)$ is the expected value of $\af(\cho{})$ when $\cho{}$ is constructed by drawing $\siz$ arms i.i.d. with replacement from $\apv$. Specifically, we first show that there exists a function $\did:2^{[\nmb]}\rightarrow\mathbb{R}$ such that for all $\bas\subseteq[\nmb]$ we have $\af(\bas)=\sum_{\ass\subseteq[\nmb]}\indi{\bas\subseteq\ass}\did(\ass)$. For all $\apv\in\mathbb{R}_+^{\nmb}$ we then define: 
\be
\phr{\af}(\apv):=\sum_{\ass\subseteq[\nmb]}\did(\ass)\left(\sum_{i\in[\nmb]}\indi{i\in\ass}\apc{i}\right)^\siz
\ee

Drawing inspiration from \textsc{Exp3} we will learn via online exponentiated gradient ascent with the functions $\phr{\ret{t}}$ using unbiased gradient estimates. Of course, this means that we must be able to construct unbiased gradient estimates. Remarkably, we show that we can use our sequence $\langle\acc{t}{j}\,|\,j\in[\siz]\rangle$ and the observed reward $\ret{t}(\cho{t})$ to construct an unbiased gradient estimate $\gra{t}$ of the function $\phr{\ret{t}}$ at $\pvt{t}$.

For exponentiated gradient ascent to work we must have that, for all trials $t$, our objective function $\phr{\ret{t}}$ is concave over the simplex. We show that a sufficient condition for this to hold is that the function $\ret{t}$ is pseudo-concave.

Now that we have all the pieces required for exponentiated gradient ascent to work, we can bound the regret with respect to any vector $\pst\in\splx{\nmb}$. i.e. we can bound the expected reward of our algorithm relative to $\sum_{t\in[T]}\phr{\ret{t}}(\pst)$. By taking $\pst$ such that $p^*_i:=\indi{i\in\ass}/|\ass|$ for some set $\ass$ we show that, given $\ret{t}$ is pseudo-submodular, we have $\phr{\ret{t}}(\ass)\geq(1-\alpha^\siz)\ret{t}(\ass)$ where $\alpha:=(|\ass|-1)/|\ass|$. By bounding the variance of the gradient estimate we show that the regret term is in $\tilde{\mathcal{O}}(\sqrt{\siz\nmb\ntr})$.

We have hence given an overview of how, when we have no costs, \alg\ works and why we require $\ret{t}$ to be pseudo-concave and pseudo-submodular. We now describe how costs are incorporated. This is done by using, instead of $\phr{\ret{t}}$, the function $\obf{t}$ defined by: 
\be
\obf{t}(\apv):=\npf{\ret{t}}(\apv)-\siz\sum_{i\in[\nmb]}\apc{i}\ctc{t}{i}
\ee
so that $\obf{t}(\pvt{t})$ lower bounds the expected profit on trial $t$. Since $\obf{t}$ differs from $\phr{\ret{t}}$ by a linear function it is straightforward to extend the above methodology to this new objective function.
